Fair Distributed Cooperative Bandit Learning on Networks for Intelligent Internet of Things Systems (Technical Report)

In intelligent Internet of Things (IoT) systems, edge servers within a network exchange information with their neighbors and collect data from sensors to complete delivered tasks. In this paper, we propose a multiplayer multi-armed bandit model for intelligent IoT systems to facilitate data collection and incorporate fairness considerations. In our model, we establish an effective communication protocol that helps servers cooperate with their neighbors. Then we design a distributed cooperative bandit algorithm, DC-ULCB, enabling servers to collaboratively select sensors to maximize data rates while maintaining fairness in their choices. We conduct an analysis of the reward regret and fairness regret of DC-ULCB, and prove that both regrets have logarithmic instance-dependent upper bounds. Additionally, through extensive simulations, we validate that DC-ULCB outperforms existing algorithms in maximizing reward and ensuring fairness.

==> sec-centralized-policy.tex <==
\section{Centralized MMAB Channel Selection Policy}
\label{sec-centralized-policy}
This section is devoted to centralized MMAB channel selection problems. Under this condition, users not only make use of other users' observations but also avoid collisions through centralized scheduling. Based on the UCB algorithm, we elaborate our channel selection algorithms for homogeneous and heterogeneous users respectively, then analyze their performance.


\subsection{Centralized UCB Algorithm for Homogeneous Users}
For the homogeneous users, the mean rewards of channels are identical across users. Hence, we aim to find the $M$ best channels with mean rewards $\left\lbrace \mu_{1},\ldots,\mu_{M} \right\rbrace $ at each time for maximizing the global reward collected by all users. Our centralized UCB algorithm for homogeneous users (\hocucb{}) considers the UCB value as an estimate of the mean reward of a channel and then selects the $M$ channels corresponding to the $M$ largest UCB values at each time. The details of the algorithm is presented in Algorithm \ref{alg:mmab:Cho-UCB}, 
\begin{algorithm}[!t]
	\KwIn{Number of users $M$, number of channels $N$}
	\KwOut{$i^{k}(t)$,$t \in \left\lbrace 1,...,T\right\rbrace  , k \in \left\lbrace 1,...,M\right\rbrace $}
	\Begin{$m_{i}(t) \leftarrow 0 , \hat{\mu}_{i}(t) \leftarrow 0 ,  i \in \left\lbrace  1,...,N \right \rbrace$}
	\For{$t=1$ \KwTo $T$}{
	\uIf{$t \leq N$}{ 
	
		$i^{k}(t) \leftarrow (k+t) \mod N +1$ ;
		\\collect $r_{i}(t)$;
		\\update $m_{i}(t)$, $ \hat{ \mu}_{i}(t)$ using \eqref{eq:mmab:sample-mean-reward} and \eqref{eq:mmab:number-of-samples}; 
		
	
	}                 % in a block unended

	   \Else{
	   \For{channel $i \in \left\lbrace  1,...,N \right \rbrace  $}{
	   $U_{i}(t) \leftarrow \hat{ \mu}_{i}(t-1) + \sqrt{\dfrac{2 \ln t}{m_{i}(t-1)}}$;
	   }	   
	   
	   		select $i^{k}(t)$ with the $k$-th largest UCB value;
	   		\\collect reward $r_{i}(t)$;
	   		\\update $m_{i}(t)$, $ \hat{ \mu}_{i}(t)$ using \eqref{eq:mmab:sample-mean-reward} and \eqref{eq:mmab:number-of-samples}; 
	   }                          % in a block
      

	   }
	  
	
	\caption{\hocucb{} algorithm at user $k$}
	\label{alg:mmab:Cho-UCB}
\end{algorithm}
where line $5$ to $7$ is the initial phase where each channel will be selected $M$ times to obtain preliminary information. $m_{i}(t)$ and $ \hat{ \mu}_{i}(t)$ are updated as follows:
\begin{equation}
\label{eq:mmab:sample-mean-reward}
 \hat{\mu}_{i}(t)=
\begin{cases}% {lll}
\dfrac{\hat{\mu}_{i}(t-1)m_{i}(t-1)+r_{i}(t)}{m_{i}(t-1)+1}       \text{,}      & {i^k(t)=i} \text{,} \\
\hat{\mu}_{i}(t-1)    \text{,}       & {\mbox{else} } \text{,}
\end{cases}
\end{equation}

\begin{equation}
\label{eq:mmab:number-of-samples}
 m_{i}(t)=% \left\{
\begin{cases}% {lll}
m_{i}(t-1)+1    \text{,}        & {i^k(t)=i} \text{,}\\
m_{i}(t-1)    \text{,}       & {\mbox{else}} \text{.}
\end{cases} % \right. 
\end{equation}


\subsection{Centralized UCB Algorithm for Heterogeneous Users}
In this section, we focus on the more challenging heterogeneous setting in which the mean reward of each channel may vary from one user to another due to different configurations and locations between users. Now, if user $k$ selects channel $i$ at time $t$, she will receive a reward with mean $\mu^k_i(t)$. Therefore, heterogeneous users can't utilize observations made by others to update their own information. Considering a bipartite graph with parts of size $M$ and $N$, we denote $\pi$ as a matching which is a one-to-one assignment of users to channels, and $\mathcal{M}$ is the set of all matchings. Moreover, the edge $(k,i)$ between user $k$ and channel $i$ has weight (mean reward) $\mu^k_i(t)$ which takes a UCB value as its estimate. Under the constraint, the target of the centralized UCB algorithm for heterogeneous users (\hecucb{}) would boil down to finding the optimal matching $\pi_t=\pi_{max}$ between users and channels which maximizes $\sum_{k=1}^{M}U^k_{\pi(k)}(t)$ at each time $t$ based on UCB algorithm. Now the system regret for \hecucb{} algorithm is redefined as 
\begin{equation}
\label{eq:mmab:Che-UCB-regret}
R^{\hecucb{}}_T=T \max_{\pi \in \mathcal{M}} \sum_{k=1}^{M} \mu^k_{\pi(k)} - \sum_{t=1}^{T} \sum_{k=1}^{M}\mu^k_{\pi_t(k)}(t) \text{.}
\end{equation}
where the optimal expected system reward is the maximum attainable total weight $\max_{\pi \in \mathcal{M}} \sum_{k=1}^{M} \mu^k_{\pi(k)}$. The details of the algorithm is presented in Algorithm \ref{alg:mmab:Che-UCB}, where we can find the optimal matching $\pi_{max}$ within polynomial time in line $13$ by the Hungarian algorithm. \cite{kuhn1955hungarian}.


\begin{algorithm}[!t]
    \label{alg:mmab:Che-UCB}
	\KwIn{Number of users $M$, number of channels $N$}
	\KwOut{$i^{k}(t)$,$t \in \left\lbrace 1,...,T\right\rbrace , k \in \left\lbrace 1,...,M\right\rbrace $}
	\Begin{$m_{i}^{k}(t) \leftarrow 0 , \hat{\mu}_{i}^{k}(t) \leftarrow 0 , k \in \left\lbrace  1,...,M,\right \rbrace,    i \in \left\lbrace  1,...,N \right \rbrace$;}
	\For{$t=1$ \KwTo $T$}{
	\uIf{$t \leq N$}{
	$i^{k}(t) \leftarrow (k+t) \mod N +1 $;
	\\collect reward $r_{i}^{k}(t)$;
	\\update $m_{i}^k(t)$, $ \hat{ \mu}^k_{i}(t)$ using \eqref{eq:mmab:sample-mean-reward} and \eqref{eq:mmab:number-of-samples};
	}                % in a block unended

	   \Else{
	   \For{channel $i \in \left\lbrace  1,...,N \right \rbrace  $}{
	   $U_{i}^{k}(t) \leftarrow \hat{\mu}_{i}^{k}(t-1) + \sqrt{\dfrac{2 \ln t}{m_{i}^{k}(t-1)}}$;
	   }  
	   	   
	   $ \pi_{\max} \leftarrow \arg \max{ \left\lbrace  \sum_{k=1}^M U^k_{\pi (k)}(t)  : \pi \in \mathcal{M} \right\rbrace   }   $; 	   
	   
	   $i^{k}(t) \leftarrow \pi_{\max}(k)$;
	   \\collect reward $r_{i}^{k}(t)$;
	   \\update $m_{i}^k(t)$, $ \hat{ \mu}^k_{i}(t)$ using \eqref{eq:mmab:sample-mean-reward} and \eqref{eq:mmab:number-of-samples};
	   
	   }                          % in a block
      

	   }
	  
	
	\caption{\hecucb{} algorithm at user $k$}
	
\end{algorithm}
\subsection{Regret Analysis of the \hocucb{} and \hecucb{} Algorithms}
The centralized MMAB channel selection problem can be regarded as a single user simultaneously selecting multiple channels at each time, also known as the combinatorial MAB problem (CMAB) \cite{gai2012combinatorial} \cite{chen2013combinatorial}. We refer to \cite{gai2012combinatorial} and get the Theorem \ref{the:mmab:expected-subopt-decisions} below.

\begin{myTheo}
\label{the:mmab:expected-subopt-decisions}
Under the centralized MMAB channel selection policy specified in Algorithm \ref{alg:mmab:Cho-UCB} and \ref{alg:mmab:Che-UCB}, the expected number of times that users make the suboptimal decisions for channel selection after $T$ time slots is at most:
\begin{equation}
\frac{8 N \ln T}{(l_{\min})^2}+N+\frac{ \pi^{2}}{3} N \text{,}
\end{equation}
\end{myTheo}
So the upper bound of system regret of the \hocucb{} and \hecucb{} algorithms in the centralized case satisfy:
\begin{equation}
%\label{cents}
\label{eq:mmab:cent-upper-bound}
%\begin{aligned}
R^{CENT}_T \leq\left[ \frac{8 N \ln T}{\left(l_{\min}\right)^{2}}+N+\frac{\pi^{2}}{3}  N\right] l_{\max}  \text{.}
%\end{aligned} 
\end{equation}
where $l_{\max}$ and $l_{\min}$ represent the maximum loss and minimum loss on the reward brought by the suboptimal decisions, respectively. We can
see that the system regret grows logarithmically in
time, which achieves order-optimal regret. 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "mmab"
%%% End:

